Regularity in time along the coarse scale flow for the incompressible Euler equations

One of the most remarkable features of known nonstationary solutions to the incompressible Euler equations is the phenomenon known as the Taylor hypothesis, which predicts that coarse scale averages of the velocity carry the fine scale features of the flow. In this work, we develop a time regularity theory for Euler weak solutions based on quantitative expressions of this hypothesis. We assume only that our velocity field is H\"{o}lder continuous in the spatial variables, which is well-motivated by problems related to turbulence, but precludes the application of Lagrangian methods or local well-posedness theory. Despite the dramatic lack of well-posedness, we obtain a rich theory of regularity in time for solutions, especially concerning advective derivatives. In particular, any Euler flow of class $v \in L_t^\infty C_x^\alpha$ has continuous advective derivatives of any order less than $\frac{\alpha}{1-\alpha}$, and every point has a trajectory passing through it that is $C^r$ for all $r < \frac{1}{1-\alpha}$, and one that is $C^\infty$ if $v$ is $C^1$ or $v \in \bigcap_{\alpha < 1} L_t^\infty C_x^\alpha$ has borderline regularity. In a follow up work, we show that all trajectories are of class $C^{1/(1-\alpha)}$ in time whenever $1/(1-\alpha) \notin {\mathbb Z}$, whether or not the trajectories are unique.

==> conclusion_old.tex <==
Several parts of the analysis in this paper give a new point of view on convex integration constructions of Euler flows and the pursuit of Onsager's conjecture.  One point which the analysis clarifies is that some of the special estimates for material derivatives in these constructions are forced by the Euler equations, rather than being artifacts of the constructions.  These bounds give another point of view on the constraints one expects for the type of scheme that could be used to approach Onsager's conjecture.  For example, the bounds on material derivatives (inequality (\ref{bd:matDvOfLpPiece2}) in particular) show that the natural time scale associated to frequency $\la \approx 2^k$ is on the order $\la^{-(1-\a)} \ctdcxa{v}^{-1}$.  In particular, any time cutoffs employed in a construction at frequency $\la$ should have a lifespan at least least $\sim \la^{-(1-\fr{1}{3})}$ in order to be compatible with the desired spatial regularity $1/3$.  The constructions of solutions in \cite{isett, deLSzeBuck} employ time cutoffs with a lifespan of size about $\la^{-(1- \fr{1}{5} + \ep)}$ and lead to regularity $v \in C_{t,x}^{1/5 - \ep}$.  However, Buckmaster has shown \cite{Buckmaster} that it is possible to obtain $C_{t,x}^{1/5-\ep}$ solutions with $v(t,\cdot) \in C_x^{1/3 - \ep}(\T^3)$ for almost every $t \in \R$.  His proof is based on the construction in \cite{deLSzeBuck} but modifies the construction while keeping careful track of the time-dependence of the estimates so that the set of ``bad times'' experiencing consistent contributions from anomalous error terms including sharp time cutoffs has measure $0$.  % (in fact, Hausdorff dimension less than $1$).  
This idea has since been upgraded in \cite{buckDeLSzeOnsCrit} to construct solutions in the class $C_{t,x}^0 \cap L_t^1 C_x^{1/3 - \ep}$.  It remains an important problem to determine if the exponent $1/5$ can be improved on in any function space that admits an advective derivative bound as in \eqref{bd:matDvOfLpPiece2} (for example, in $L^2$ based function spaces $L_t^2 H^{1/5 + \ep}$).

%His proof is based on the construction in \cite{deLSzeBuck}, but modifies the construction and keeps careful track of the time-dependence of the estimates in order to ensure that the set of ``bad times'' on which the solutions possess lower regularity turns out to have measure $0$ (in fact, Hausdorff dimension less than $1$).  

%His proof is based on the construction in \cite{deLSzeBuck} but keeps careful track of the time-dependence of the estimates and modifies the construction so that the set of ``bad times'' which experience consistent contributions from anomalous error terms including the harmful time cutoffs has measure $0$ (in fact, Hausdorff measure less than $1$).

Theorem \ref{thm:energyReg} on the regularity of the total energy suggests some further questions regarding the energy profiles of Euler flows.  De Lellis and Sz\'{e}kelyhidi have shown \cite{deLSzeHoldCts} that the energy profile of an Euler flow constructed by convex integration can be essentially any smooth, positive function (see also \cite{deLSzeBuck}).  Refinements of this result tailored to the initial value problem show that uniqueness for the initial value problem for the Euler equations in H\"{o}lder spaces cannot be restored by many natural ``entropy criteria'' one might propose (see \cite{deLSzeAdmiss, Daneri}). There is a restriction in \cite{deLSzeHoldCts, deLSzeBuck} that the energy profile is bounded below by a positive constant, but this restriction may be purely technical.  It is reasonable to suspect that the energy profile can also be made rough as well, and it would be interesting to see whether the regularity in Theorem (\ref{thm:energyReg}) is sharp since the proof of Theorem (\ref{thm:energyReg}) is closely related to the proof of energy conservation in \cite{CET}.  For exponents $\a < 1/5$, the sharpness of regularity for the energy profile has now been proven in \cite{isettOhNonpd}.  %(This result would simultaneously exhibit that the velocity fields obtained from the construction are indeed no better than the claimed exponent.)

It would be of further interest to show that irregularity of the energy profile is a generic behavior for solutions with regularity strictly below $1/3$.  That is, for an Euler flow which is generic in a space similar to $C_tC_x^\a$ with $\a < 1/3$, we expect that the energy profile will not belong to any space with better regularity than $C_t^{\fr{2 \a}{1 - \a}}$, and furthermore should fail to be of bounded variation on every time interval.  In particular, a small perturbation of Euler flows in $C_tC_x^\a$ for $\a < 1/3$ should generically lead to an irregular energy profile which does not consistently decrease or increase on any time interval, in contrast to the discussion of the case $\a = 1/3$ in Section~\ref{sec:timeRegEnergy}.  Such a result would indicate that energy dissipation at regularity below $1/3$, while possible, is an unstable phenomenon, so that the $1/3$ law \eqref{law:oneThird} would be the only possible law for velocity fluctuations that is compatible with the dissipation of energy in a robust sense.  See \cite{isettOhNonpd} for results in support of this conjecture in the range $\a < 1/5$. %In the regime $\a < 1/5$ might be approachable by the methods of convex integration.% since a general Euler flow can be smoothed to obtain an Euler Reynolds flow, but for this application we may need a bound such as (\ref{ineq:bdForDdtRleqk}) which is valid in the regime $\a < 1/3$.


\begin{comment}
Several of the results of this paper indicate that the fundamental bounds satisfied by the solutions to the Euler equations constructed by convex integration are actually common to general weak solutions of the Euler equations with H\"{o}lder regularity.  In particular, it is clear that the advective derivative obeys estimates which are superior to those satisfied by the time derivative.  These results give some justification to the heuristic suggested in \cite{isett} that the Euler-Reynolds flows $(v, p, R)$ in convex integration behave like low frequency projections of solutions to the Euler equations.  To be more precise, the velocity $v_{(k)}$ should behave like $P_{\leq k} v$, but the pressure does not behave like $P_{\leq k} p$ in that one continues to add low frequency corrections to the pressure $p$ during the entire process, so the pressure $p$ in convex integration seems to be more closely analogous to the $p_{(k)}$ in the present proof.  Regarding the validity of this heuristic, it is worth noting we have not achieved the bounds
\ali{
 \co{ \nab^A (\pr_t + P_{\leq k} v \cdot \nab) R_{\leq k} } &\leq 2^{(A + (1-\a) - 2 \a) k} \ctdcxa{v}^3  \label{eq:basicStressBoundEnd} \\
\co{ \nab^A (\pr_t + P_{\leq k} v \cdot \nab) \nab P_{\leq k} p } &\leq 2^{(A + (1-\a) + 1 - 2 \a) k} \ctdcxa{v}^3  \label{eq:basicPressBoundEnd}
}
without the restriction $\a > 1/3$.  The bound (\ref{eq:basicStressBoundEnd}) for the Reynolds stress in convex integration plays a fundamental role in the construction of solutions.  It would be of interest to show that a frequency projected velocity field $P_{\leq k} v$ (or some similar approximation to $v$) satisfies the Euler Reynolds equations with a stress which obeys the bound (\ref{eq:basicStressBoundEnd}).
\end{comment}
